InfoNCE: Identifying the Gap Between Theory and Practice

Prior theory work on Contrastive Learning via the InfoNCE loss showed that, under certain assumptions, the learned representations recover the ground-truth latent factors. We argue that these theories overlook crucial aspects of how CL is deployed in practice. Specifically, they either assume equal variance across all latents or that certain latents are kept invariant. However, in practice, positive pairs are often generated using augmentations such as strong cropping to just a few pixels. Hence, a more realistic assumption is that all latent factors change with a continuum of variability across all factors. We introduce AnInfoNCE, a generalization of InfoNCE that can provably uncover the latent factors in this anisotropic setting, broadly generalizing previous identifiability results in CL. We validate our identifiability results in controlled experiments and show that AnInfoNCE increases the recovery of previously collapsed information in CIFAR10 and ImageNet, albeit at the cost of downstream accuracy. Finally, we discuss the remaining mismatches between theoretical assumptions and practical implementations.

==> Tables/causal_3dident.tex <==
\begin{table*}[tb]
%\setlength{\tabcolsep}{2pt}
\footnotesize
\centering
\caption{
    \textbf{We observe the accuracy-identifiability trade-off on C-3DIdent for views generated by Color augmentations.}
In that case, while InfoNCE achieves better accuracy, \ourloss has higher $R^2$ scores. In all other settings, \ourloss outperforms InfoNCE in terms of both accuracy and identifiability scores. We report averaged results over three random seeds and the standard deviation.
}
 \label{tab:3dident}

\newcolumntype{h}{>{\columncolor[gray]{0.9}}c}
\newcolumntype{i}{>{\columncolor[gray]{0.85}}c}
\setlength\tabcolsep{2pt} % default value: 6pt

\begin{NiceTabular}{l| cc cc |cc cc }[colortbl-like]
\toprule
%\multicolumn{1}{c}{Training Objective} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Features} & \multicolumn{1}{c}{Grayscale} & \multicolumn{1}{c}{Brightness} & \multicolumn{1}{c}{Contrast} & \multicolumn{1}{c}{Hue} & \multicolumn{1}{c}{Saturate} & \multicolumn{1}{c}{Avg.} \\
& \multicolumn{4}{c}{Color} & \multicolumn{4}{c}{Crop}\\
& \multicolumn{2}{h}{Augmentations}& \multicolumn{2}{h}{DGP} &  \multicolumn{2}{c}{Aug. (Large)}&\multicolumn{2}{c}{DGP} \\
Loss & Class & $R^2$ & Class & $R^2$ & Class & $R^2$ & Class & $R^2$\\
 \midrule
  InfoNCE & \textbf{0.53{\fontsize{1.5}{4}\selectfont $\pm0.048$}} & 0.33{\fontsize{1.5}{4}\selectfont $\pm0.021$}
  &
  0.87{\fontsize{1.5}{4}\selectfont $\pm0.188$} & 0.67{\fontsize{1.5}{4}\selectfont $\pm0.184$}
  &
 \textbf{0.59}{\fontsize{1.5}{4}\selectfont $\pm0.01$} & 0.44{\fontsize{1.5}{4}\selectfont $\pm0.011$}
 &
 0.88{\fontsize{1.5}{4}\selectfont $\pm0.17$} & 0.8{\fontsize{1.5}{4}\selectfont $\pm0.155$}
  \\
AnInfoNCE &
0.5{\fontsize{1.5}{4}\selectfont $\pm0.003$} & \textbf{0.34}{\fontsize{1.5}{4}\selectfont $\pm0.01$}
&
\textbf{1.0}{\fontsize{1.5}{4}\selectfont $\pm0.001$} & \textbf{0.81}{\fontsize{1.5}{4}\selectfont $\pm0.003$}
&
\textbf{0.59}{\fontsize{1.5}{4}\selectfont $\pm0.02$} & \textbf{0.46}{\fontsize{1.5}{4}\selectfont $\pm0.026$}
&
\textbf{1.0}{\fontsize{1.5}{4}\selectfont $\pm0.0$} & \textbf{0.92}{\fontsize{1.5}{4}\selectfont $\pm0.001$}
\\
% InfoNCE & \textbf{0.53} & 0.33 & 0.99 & 0.79 & \textbf{0.57} & 0.43& \textbf{1.0} & 0.91 \\
% \ourloss & 0.51 & \textbf{0.34} & \textbf{1.0} & \textbf{0.80} & 0.53 & \textbf{0.46} & \textbf{1.0} & \textbf{0.92}\\
\bottomrule
\end{NiceTabular}



\end{table*}

